Infinity Search: Approximate Vector Search with Projections on q-Metric Spaces

An ultrametric space or infinity-metric space is defined by a dissimilarity function that satisfies a strong triangle inequality in which every side of a triangle is not larger than the larger of the other two. We show that search in ultrametric spaces with a vantage point tree has worst-case complexity equal to the depth of the tree. Since datasets of interest are not ultrametric in general, we employ a projection operator that transforms an arbitrary dissimilarity function into an ultrametric space while preserving nearest neighbors. We further learn an approximation of this projection operator to efficiently compute ultrametric distances between query points and points in the dataset. We proceed to solve a more general problem in which we consider projections in $q$-metric spaces -- in which triangle sides raised to the power of $q$ are smaller than the sum of the $q$-powers of the other two. Notice that the use of learned approximations of projected $q$-metric distances renders the search pipeline approximate. We show in experiments that increasing values of $q$ result in faster search but lower recall. Overall, search in q-metric and infinity metric spaces is competitive with existing search methods.

==> IMAGES/10_vp_tree.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variable to scale the plot. Modify \myfactor only.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\myfactor{1.30}  \def\unit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some tikz styles that we use in this plot
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{DotColor}{HTML}{FF0000}
\definecolor{TangentColor}{HTML}{FF0000}

\tikzstyle {dot} = [circle, fill = DotColor, opacity = 1.0, inner sep = 1pt]
\tikzstyle {tangent} = [draw, TangentColor, opacity = 1.0, line width = 0.5pt]
\tikzstyle {vector} = [tangent, -stealth]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Global Plot Definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathsetmacro{\vpx}{0}    % Vantage point v, x coordinate
\pgfmathsetmacro{\vpy}{0}    % Vantage point v, y coordinate
\pgfmathsetmacro{\vpmu}{2.5} % Radius mu at current vantage point


\pgfmathsetmacro{\nrpointsindataset}{200} % Number of points in the dataset

\pgfmathsetmacro{\xclipleft} {\vpx - 1.2*\vpmu} % Clip on the x axis left
\pgfmathsetmacro{\xclipright}{\vpx + 2.3*\vpmu} % Clip on the y axis right
\pgfmathsetmacro{\yclipbelow}{\vpy - 0.2*\vpmu} % Clip on the y axis below
\pgfmathsetmacro{\yclipabove}{\vpy + 1.2*\vpmu} % Clip on the y axis above

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{

\fontsize{8}{8} \selectfont

\begin{tikzpicture}[x = 1.0*\unit, y = 1.0*\unit] 

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Clip to remove irrelevant part of the plot

    \clip (\xclipleft,\yclipbelow) rectangle (\xclipright,\yclipabove);


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % REPRESENTATION OF THE DATASET, THE VANTAGE POINT, AND THE MEDIAN DISTANCE MU
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Add green random points to represent the dataset. Draw a green background for the whole space. 
        % Remove the circle defined by v and mu

        \foreach \i in {1,...,\nrpointsindataset}
        {
            \pgfmathsetmacro{\randpointx}{0.05 + \xclipleft  + 0.95*abs(rand)*(\xclipright-\xclipleft)}        
            \pgfmathsetmacro{\randpointy}{0.05 + \yclipbelow + 0.95*abs(rand)*(\yclipabove-\yclipbelow)}        
            \path (\randpointx,\randpointy) node [dot, fill = mygreen!10] {};            
        }

        \path[fill = mygreen, opacity = 0.2] 
            (\xclipleft,\yclipbelow)  -- (\xclipright,\yclipbelow) --
            (\xclipright,\yclipabove) -- (\xclipleft,\yclipabove) -- cycle;

        \path (\vpx, \vpy) 
            node [circle, fill = white, minimum width = 2*\vpmu*\unit] {};
            
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw blue random points to represent the dataset. Draw a circle to represent the points in the 
        % dataset that are closer than \mu to the vantage point. 

        \foreach \i in {1,...,\nrpointsindataset}
        {
            \path (rand*180: rand*\vpmu) node [dot, fill = blue!10 ] {};
        }

        \path (\vpx, \vpy) 
            node [circle, fill = blue, opacity = 0.2, minimum width = 2*\vpmu*\unit] {};


        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw the vantage point v and a circle centered at the vantage point with radius mu
        \path (\vpx, \vpy) 
            node [circle, minimum width = 2*\vpmu*\unit, draw = black!50, thick] {}
            node [dot,    fill = blue] (v) {}
            node [below left] {$v$};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % REPRESENTATION OF A POINT THAT REQUIRES EXPLORATION OF THE INTERIOR OF THE VP TREE ONLY
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \pgfmathsetmacro{\xd}{1.3}     % Point x, distance from vantage point
        \pgfmathsetmacro{\xa}{155}   % Point x, angle from vantage point
        \pgfmathsetmacro{\xtau}{0.8} % Point x, distance to current best point

        \pgfmathsetmacro{\ua}{45}  % Point u, angle from Point x

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw the point x and a circle centered at x with radius tau
        \path (v) ++ (\xa:\xd)
            node [circle, fill = red, opacity = 0.2, minimum width = 2*\xtau*\unit, draw = red] {}
            node [dot,    fill = red] (x) {}
            node [below left] {$x_0$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw point u which is the current closest to x
        \path (x) ++ (\ua:\xtau) 
            node [dot, fill = red] (u) {}
            node [above right] {$u$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw and annotate lines connecting v to x and x to u
        \path [draw] (v) -- (x) node [midway, above] {$~~~~~d(x_0,v)~$};
        \path [draw] (x) -- (u) node [midway, left] {$d(x_0,u)~$};

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % REPRESENTATION OF A POINT THAT REQUIRES EXPLORATION OF THE EXTERIOR OF THE VP TREE ONLY
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \pgfmathsetmacro{\xd}{3.8}     % Point x, distance from vantage point
        \pgfmathsetmacro{\xa}{22}   % Point x, angle from vantage point
        \pgfmathsetmacro{\xtau}{0.9} % Point x, distance to current best point

        \pgfmathsetmacro{\ua}{-45}  % Point u, angle from Point x

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw the point x and a circle centered at x with radius tau
        \path (v) ++ (\xa:\xd)
            node [circle, fill = red, opacity = 0.2, minimum width = 2*\xtau*\unit, draw = red] {}
            node [dot,    fill = red] (x) {}
            node [above right] {$x_0'$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw point u which is the current closest to x
        \path (x) ++ (\ua:\xtau) 
            node [dot, fill = red] (u) {}
            node [below] {$u'$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw and annotate lines connecting v to x and x to u
        \path [draw] (v) -- (x) node [midway, below] {$~~~~d(x_0',v)~$};
        \path [draw] (x) -- (u) node [midway, right] {$~d(x_0',u')$};
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % REPRESENTATION OF A POINT THAT REQUIRES EXPLORATION OF BOTH SIDES OF THE VP TREE
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \pgfmathsetmacro{\xd}{0.9*\vpmu}     % Point x, distance from vantage point
        \pgfmathsetmacro{\xa}{70}   % Point x, angle from vantage point
        \pgfmathsetmacro{\xtau}{0.6} % Point x, distance to current best point

        \pgfmathsetmacro{\ua}{45}  % Point u, angle from Point x

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw the point x and a circle centered at x with radius tau
        \path (v) ++ (\xa:\xd)
            node [circle, fill = red, opacity = 0.2, minimum width = 2*\xtau*\unit, draw = red] {}
            node [dot,    fill = red] (x) {}
            node [above left] {$x_0''$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw point u which is the current closest to x
        \path (x) ++ (\ua:\xtau) 
            node [dot, fill = red] (u) {}
            node [above right] {$u''$};

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Draw and annotate lines connecting v to x and x to u
        \path [draw] (v) -- (x) node [midway, right] {$~~~~d(x_0'',v)~$};
        \path [draw] (x) -- (u) node [midway, right] {$~d(x_0'',u'')$};
   
   
\end{tikzpicture}

}
